Self-Configuring nnU-Nets Detect Clouds in Satellite Images

Cloud detection is a pivotal satellite image pre-processing step that can be performed both on the ground and on board a satellite to tag useful images. In the latter case, it can help to reduce the amount of data to downlink by pruning the cloudy areas, or to make a satellite more autonomous through data-driven acquisition re-scheduling of the cloudy areas. We approach this important task with nnU-Nets, a self-reconfigurable framework able to perform meta-learning of a segmentation network over various datasets. Our experiments, performed over Sentinel-2 and Landsat-8 multispectral images revealed that nnU-Nets deliver state-of-the-art cloud segmentation performance without any manual design. Our approach was ranked within the top 7% best solutions (across 847 participating teams) in the On Cloud N: Cloud Cover Detection Challenge, where we reached the Jaccard index of 0.882 over more than 10k unseen Sentinel-2 image patches (the winners obtained 0.897, whereas the baseline U-Net with the ResNet-34 backbone used as an encoder: 0.817, and the classic Sentinel-2 image thresholding: 0.652).

==> new_commands.tex <==
% General (SVM) symbols
\newcommand{\TrainingSample}{\bm{t}} % OK
\newcommand{\InputSample}{\bm{x}} % OK
\newcommand{\WeightVector}{\bm{w}} % OK
\newcommand{\MaximumMargin}{\varphi} % OK
\newcommand{\Bias}{b} % OK
\newcommand{\ClassLabel}{y} % OK
\newcommand{\InputDimensionality}{\mathcal{D}} % OK
\newcommand{\DataMatrix}{\mathcal{D}}
\newcommand{\CovarianceMatrix}{\mathcal{C}}
\newcommand{\RealSet}{\mathbb{R}^{\rm \mathcal{D}}} % OK
\newcommand{\RealSetBands}{\mathbb{R}^{b}} % OK
\newcommand{\RealValue}{\mathbb{R}} % OK
\newcommand{\ClassA}{C_{+}} % OK
\newcommand{\ClassB}{C_{-}} % OK
\newcommand{\Slack}{\xi} % OK
\newcommand{\KernelMap}{\phi} % OK
\newcommand{\PenaltyParameter}{C} % OK
\newcommand{\KernelFunction}{\mathcal{K}} % OK
\newcommand{\FeatureSpace}{\mathbb{F}} % OK
\newcommand{\LagrangeMultiplier}{\alpha} % OK
\newcommand{\SVMTrainingTimeComplexity}{O(\TrainingSetSize^3)}
\newcommand{\SVMTrainingMemoryComplexity}{O(\TrainingSetSize^2)}
\newcommand{\PolynomialDegree}{l} % OK
\newcommand{\SigmoidBias}{\kappa} % OK
\newcommand{\Lagrangian}{\mathcal{L}} % OK
\def\sgn{\mathop{\rm sgn}\nolimits}

% Fuzzy kernel symbols
\newcommand{\NumberOfFuzzyRules}{L_{f}} % OK
\newcommand{\FuzzyRule}{l_{f}} % OK
\newcommand{\fuzzyImplication}{\rightsquigarrow} % OK
\newcommand{\term}[1]{\mathfrak{#1}}
\newcommand{\zbior}[1]{\mathbb{#1}}  % set
\newcommand{\macierz}[1]{{\boldsymbol{\mathrm{#1}}}}
\newcommand{\wektor}[1]{\macierz{\MakeLowercase{#1}}}
\newcommand{\newItem}[2]{%
  \expandafter\def\csname #1\endcsname {\MakeLowercase{#2}} %
  \expandafter\def\csname n#1\endcsname {\MakeUppercase{#2}} %
  \expandafter\def\csname zb#1\endcsname {\zbior{\MakeUppercase{#2}}} %
  \expandafter\def\csname t#1\endcsname {\term{\MakeLowercase{#2}}} %
  \expandafter\def\csname m#1\endcsname {\macierz{\MakeUppercase{#2}}} %
  \expandafter\def\csname w#1\endcsname {\wektor{#2}} %
  }
  \newItem{Atrybut}{d_f}
\newItem{Deskryptor}{x}
\newItem{Regula}{l}
\newItem{Przeslanka}{a}
\newItem{Konsekwencja}{b}
\newItem{Implikacja}{b'}
\newItem{Zespolona}{c}
\newItem{Rzeczywista}{r}
\newItem{Klasa}{\delta}
\newItem{Decyzja}{y}
\newItem{Przyklad}{a}
\newItem{Test}{a}
\newItem{Klaster}{c}
\newItem{Rozmycie}{s}
\newItem{Centre}{v}
\newItem{Membership}{u}
\newItem{ClusterMembership}{\mu}
\newItem{Weight}{z}
\newItem{Krotka}{x}
\newItem{Width}{w}
\newItem{Wspolczynnik}{p}
\newItem{Obiekt}{k}
\newItem{Odleglosc}{t}
\newItem{Parameter}{p}
\newcommand{\reg}{^{(\Regula)}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\tr}{^{\T}}

% operatory
%\DeclareMathOperator*{\tnorm}{\star}
%\DeclareMathOperator*{\opBigTnorm}{\bigstar}
%\newcommand{\bigtnorm}[2]{\opBigTnorm\limits^{#2}_{#1}}
%% \newcommand{\tNormOp}[2]{#1 \tnorm #2}
%\newcommand{\tNormOp}[2]{T \left(#1, #2\right)}
%\DeclareMathOperator{\abs}{\mathrm{sgn}}
%\newcommand{\firStr}{F} % firing strength
%\newcommand{\w}[1]{\macierz{#1}}
%
%\newcommand{\localisation}{y}
%\newcommand{\SystemAnswer}{\localisation_0}
%\newcommand{\kernelNFSEXP}{NFS-exponential}
%\newcommand{\kernelNFSPROD}{NFS-product}

% General (algorithm) symbols
\newcommand{\ChromosomeHalfSize}{K} % OK
\newcommand{\Generation}{G} % OK
\newcommand{\NumberOfGenerations}{g} % OK
\newcommand{\PopulationSize}{N} % OK
\newcommand{\Fitness}{\eta} % OK
\newcommand{\FitnessForValidationSet}{\eta_{\ValidationSet}} % OK
\newcommand{\Individual}{p}
\newcommand{\TrainingSet}{\bm{T}} % OK
\newcommand{\TrainingSetSize}{N}
\newcommand{\ValidationSet}{\bm{V}} % OK
\newcommand{\ValidationSetSize}{v}
\newcommand{\TestSet}{\Psi} % OK
\newcommand{\TestSetSize}{\psi}
\newcommand{\ElliteSize}{\epsilon}
\newcommand{\RefinedTrainingSet}{\bm{T'}}
\newcommand{\RefinedTrainingSetSize}{t'}
\newcommand{\RefinedTrainingSetASize}{t'_{+}}
\newcommand{\RefinedTrainingSetBSize}{t'_{-}}
\newcommand{\RefinedTrainingIthSet}{\bm{T'_{i}}} % OK
\newcommand{\BestIndividual}{p^B} % OK
\newcommand{\NumberOfSupportVectors}{s}
\newcommand{\AveragePopulationFitness}{\bar{\eta}} % OK
\newcommand{\MutationProbability}{\mathcal{P}_m} % OK
\newcommand{\CrossoverProbability}{\mathcal{P}_c} % OK
\newcommand{\MaxExecutionTime}{\tau_M} % OK
\newcommand{\MaxNumberOfGenerations}{g_{\rm max}} % OK
\newcommand{\ConvergenceTime}{\tau_{c}} % OK
\newcommand{\PercentageOfSVsInIndividual}{\varrho_{SV}}

% GASVM symbols
\newcommand{\GASVMRegenerationCoefficient}{c_{g}}
\newcommand{\GASVMHLFCoefficient}{c_{h}}
\newcommand{\GASVMTruncationCoefficient}{c_{t}}
\newcommand{\GASVMEnhancedTruncationCoefficient}{c_{e}}
\newcommand{\GASVMReproductionCoefficient}{c_{r}}
\newcommand{\GASVMRestoringCoefficient}{c_{c}}
\newcommand{\GASVMMinimumImprovementThreshold}{\epsilon_{I}}
\newcommand{\GASVMMaximumStableBestFitnessCounter}{s_{b}}
\newcommand{\GASVMMaximumStableAverageFitnessCounter}{s_{a}}
\newcommand{\GASVMMaximumNumberOfRegenerations}{r}

% AGA symbols
\newcommand{\AGAInitialK}{K_i} % OK
\newcommand{\AGAPreviousK}{K^P}
\newcommand{\AGACounterWithoutBestFitnessIncrease}{c_B} % OK
\newcommand{\AGACounterWithoutAverageFitnessIncrease}{c_A} % OK
\newcommand{\AGADistanceBetweenIndividuals}{\rho} % OK
\newcommand{\AGASimilarity}{S} % OK
\newcommand{\AGAIndicesHistogram}{H}
\newcommand{\AGAHistogramBin}{h}
\newcommand{\AGAIntervalEndpoint}{C}
\newcommand{\AGAInitialPopulationSize}{N_i}
\newcommand{\AGAPopulationGrowthFactor}{\omega}
\newcommand{\AGAMaxNumberOfRegenerationsWithGrow}{R}
\newcommand{\AGAMaxNumberOfRegenerationsWithoutGrow}{R^C}
\newcommand{\AGAKIncreaseFactor}{\mu}
\newcommand{\AGAPopulationSizeIncreaseFactor}{\omega}
\newcommand{\AGAPCADimensionality}{d} % OK
\newcommand{\AGAPCAIthIntervals}{\mathcal{C}^{(i)}} % OK
\newcommand{\AGAPCAIntervals}{\mathcal{C}} % OK
\newcommand{\AGAEigenvector}{\bm{e}}
\newcommand{\AGAEigenvalue}{\lambda}
\newcommand{\AGAPopulationDiversity}{\phi}
\newcommand{\AGAFitnessDeviationOfBestIndividual}{\sigma_\Fitness}
\newcommand{\AGAPopulationDiversityDeviation}{\sigma_P}
\newcommand{\AGANumberOfGenerationsWithPopulationDiversity}{s_\phi}
\newcommand{\AGAMinimumDistanceBetweenIndividualsForTournament}{d_m}
\newcommand{\AGASteadyStateFlag}{u_B}

% DAGA symbols
\newcommand{\DAGABestFitnessBeforeIncrease}{\eta_I}
\newcommand{\DAGABestFitnessInPreviousGeneration}{\eta_P}
\newcommand{\DAGAStableChromosomeCounter}{c_s}
\newcommand{\DAGATotalImprovement}{\Delta_T}
\newcommand{\DAGARecentImprovement}{\Delta_R}
%\newcommand{\DAGASVRatio}{\varrho_{SV}}
\newcommand{\DAGASVRatioThreshold}{\mathcal{T}_{\rm SV}}
\newcommand{\DAGAIncreaseFactor}{\delta_K}
\newcommand{\DAGAStableChromomosmeLimit}{\mathcal{T}_s}

% MASVM symbols
\newcommand{\MASVMSVPoolSize}{t^s} % OK
\newcommand{\MASVMSupportVectorsPool}{\bm{P}} % OK
\newcommand{\MASVMEducationProbability}{\mathcal{P}_e} % OK
\newcommand{\MASVMLGACoefficient}{\epsilon_{\rm LGA}} % OK
\newcommand{\MASVMPercentageOfSIs}{\chi} % OK

% PCAAMA symbols
\newcommand{\PCAAMAAlgorithmName}{PCA$^2$MA}
\newcommand{\PCAAMAValuableSamplesSetSize}{t^c} % OK
\newcommand{\PCAAMAValuableSamplesSet}{\bm{T^c}} % OK
\newcommand{\PCAAMAValuableSamplesSetA}{\bm{T^c_{+}}}
\newcommand{\PCAAMAValuableSamplesSetB}{\bm{T^c_{-}}}
\newcommand{\PCAAMAPCATime}{\tau_{\rm PCA}} % OK
\newcommand{\PCAAMAPercentageOfRemovedSamplesFromCluster}{\zeta} % OK
\newcommand{\PCAAMAKIncrement}{\Delta_K}
\newcommand{\PCAAMAAverageNumberOfSVs}{\bar{s}}
%\newcommand{\PCAAMAMaxMATime}{\tau_{\rm MA}} % OK

% Experimental validation symbols
\newcommand{\QualityFunction}{Q}
\newcommand{\QualityImportanceFunction}{q} 
